Surveying Uncertainty Representation: A Unified Model for Cyber-Physical Systems

Cyber-Physical Systems (CPS) operate in dynamic environments, leading to different types of uncertainty. This work provides a comprehensive review of uncertainty representations and categorizes them based on the dimensions used to represent uncertainty. Through this categorization, key gaps and limitations in existing approaches are identified. To address these issues, a Conceptual Model of Uncertainty Representations in CPS is introduced, integrating and extending existing models. Its applicability is demonstrated through examples from the automotive domain, showing its effectiveness in capturing and structuring uncertainty in real-world scenarios.

==> chapters/Background.tex <==
\section{Background}~\label{sec:background}


==> chapters/Future_Directions.tex <==
\section{Future Directions}
\label{sec:futureDirections}

\paragraph{Domain-specific Extension}
Classification of sources ,
other specific ``entities'' that we leave \{Applications}
CONVIDE  ... 



==> chapters/RelatedLiterature/location_old.tex <==
\subsection{Location}~\label{sec:location}
%A total of nine papers address a category concerning the location of uncertainty in the representation of uncertainty. 
%In the following paragraphs, we will explore the various definitions of uncertainty location.
Walker et al.~\cite{walker2003defining} define the location of uncertainty as the point of manifestation within a complex model.
%identification of where the uncertainty manifests itself within the model complex. 
%The location description in the model will vary according to the considered system model. 
Ideally, location description helps identify where the uncertainty affecting the outcome is created in the model.
Walker et al. list some typical locations that can be applied to most models: \textit{Context, Model, Inputs, Parameter, and  Outcome}.
\textit{Context} identifies the system's boundaries, defining what is inside and outside and how fully it represents the real world.
The conceptual model, which defines the variables and relationships within the system, and the computer model are both associated with \textit{Model} uncertainty.
Model uncertainty can be divided into model structure uncertainty concerning the model's form and technical uncertainty related to its computer implementation.
\textit{Inputs} are related to the description of the reference system, often the current system, and the external forces driving its changes.
The data and the methods to calibrate the model parameters are associated with \textit{Parameter} uncertainty. 
%\textit{Parameter Uncertainty} refers to the data and the methods used to calibrate the model parameters
Uncertainty related to the difference between model outcomes and true values, when significant to the decision-maker, is referred to as \textit{Outcome} uncertainty.
%Uncertainty related to the model outcomes that are significant to the decision-maker is referred to as \textit{Model outcome uncertainty}.
Chipman et al.~\cite{chipman2015coverage} base their definition of uncertainty location on the definition of Walker et al.~\cite{walker2003defining}, yet they choose a slightly different categorization with three types: \textit{Input}, \textit{Parameters}, and \textit{Models}.
%Categories for the Location of an Uncertainty presented by \citetitle{chipman2015coverage} are \textit{Input-, Parameters-, and Modeling Uncertainties}. 
\textit{Input} uncertainties are usually caused by the lack of knowledge of initial operating conditions or unforeseen scenarios. 
In cases where accurate values are unknown are modeled as \textit{Parameter} uncertainties. 
For some of these values, statistical knowledge or a range from which the values are chosen is available.
\textit{Model} uncertainty refers to uncertainties regarding the representation of an existing system.


The taxonomy by Perez-Palacin et al.~\cite{perez2014uncertainties} 
%define the point within a model where uncertainty manifests as the location of uncertainty.
%The location of uncertainty is described by Perez-Palacin et al.~\cite{perez2014uncertainties} as the point within the model where uncertainty manifests.
%The presented options for the 
presents three types of location of uncertainty   \textit{Context}, \textit{Model structural}, and \textit{Input}. 
Although these terms are covered by Walker et al.~\cite{walker2003defining}, they have different meanings in this taxonomy. 
\textit{Context uncertainty} concerns the completeness of the model with respect to the real world, and \textit{Model structural uncertainty} represents how accurately the model represents the modeled subset of the real world. %, the less Model structural uncertainty exists. 
\textit{Input}, also called parameter, refers to uncertainty concerning the actual values of input variables in the model or calibrating methods. %given as input to the model or variable calibrating methods.

Pelz et al.~\cite{pelz2021mastering} introduce the category \textit{System Design} to identify where uncertainties occur, covering: \textit{Model} uncertainty as defined by Chipman et al.~\cite{chipman2015coverage}, \textit{Structural} similar to Perez-Palacin~\cite{perez2014uncertainties}, and \textit{Data} uncertainty. 
\textit{Data} uncertainty arises when there is a lack of completeness, clarity, or sufficiency in the required data's amount, type, or distribution.
%\textit{Structural Uncertainty} refers to the insufficient understanding of various possible function structures and the elements that generate them.

%\subsubsection{\citetitle{perez2014uncertainties}}

%\subsubsection{\citetitle{acosta2022uncertainty}}

The two understandings of Pelz et al.~\cite{pelz2021mastering} and Perez-Palacin et al.~\cite{perez2014uncertainties} about the location of uncertainty are combined by Acosta et al. ~\cite{acosta2022uncertainty} into a new notion called \textit{locus}.
\textit{Locus} specifies which model elements are affected (locus) and the `location in the real world.'
The different categories of the locus of uncertainty are \textit{Parameters}, \textit{Models}, \textit{Analysis}, and \textit{Decision Making}. 
\textit{Parameter} includes uncertainties related to all types of parameters that characterize a model.
Uncertainty related to the model definition, formalism selection, boundaries, and structure are combined in the category \textit{Models}.
The category \textit{Analysis} comprises uncertainty from evaluating design decisions through model-based methods. 
%This uncertainty arises from model abstractions and may be exacerbated by inaccuracies in analysis algorithms, such as approximations.
Uncertainties in the category \textit{Decision-Making} relate to the decision-making process when different options are available or when the decision is based on incomplete information and only estimates of the values of interest are available.


%\subsubsection{\citetitle{walker2003defining}}
%In their work, 
%\textit{Model uncertainty} arises from both the conceptual model, which defines the variables and relationships within the system, and the computer model. 

%\subsubsection{\citetitle{chipman2015coverage}}


%\subsubsection{\citetitle{mahdavi2017classification}}
Mahdavi-Hezavehi et al.~\cite{mahdavi2017classification} define the location of uncertainty as the specific location within the whole system where uncertainty manifests.
Possible locations for uncertainty include \textit{Environment, Model, Adaption functions, Goals, Managed systems, and Resources}. 
\textit{Environment} includes the execution context and humans interacting with or affecting the system.
\textit{Model} refers to various conceptual models representing the system. 
Functionalities performed as part of MAPE-K~\cite{kephart2003vision} are referred to as the option \textit{Adaptation functions}. 
The specification, modeling, and alternation of system goals are grouped under \textit{Goals}. 
All application-specific monitoring and adaptation systems are organized as option \textit{Managed Systems}.
\textit{Resources} refers to various essential factors and components the self-adaptive system requires to operate normally.


%\textit{Model outcome uncertainty} refers to uncertainty related to the model outcomes of interest to the decision-maker.

Other works do not further categorize the locations of uncertainty, but provide constructs in their model to represent it. 
Zhang et al.\cite{zhang2016understanding} propose a Belief Model, where the location of uncertainty is defined in the Uncertainty Model as the particular place or position where uncertainty occurs in such a Belief Statement. 
Bandyszak et al.~\cite{bandyszak2020orthogonal} present an Uncertainty Ontology and use the term \textit{Observation Point}  to document the artifacts that contain uncertainty and serve as locations where the system can detect this uncertainty.
Each observation point may be associated with multiple data sources, which represent multiple locations for uncertainty.

==> chapters/RelatedLiterature/source_old.tex <==
\subsection{Source}\label{sec:source}
In our selected literature, Ramirez et al.~\cite{ramirez2012taxonomy} provide the first description of Uncertainty Sources focusing on dynamically adaptive systems. 
This work identifies 26 distinct sources of uncertainty, categorized in three phases in the model lifecycle: \textit{Requirement Level}, \textit{Design-Time}, and \textit{Run-Time}.\\
Esfahani et al.~\cite{esfahani2013uncertainty} uses a reference architecture for self-adaptive software systems called FORMS~\cite{weyns2010forms} to determine sources of uncertainty. % in the domain of self-adaptive systems.
FORMS breaks a self-adaptive system (SAS) into four different components: the User, the Environment, the Base-Level -- which includes the main functionalities of the system -- and the Meta-Level, which manages the Base-Level's behavior using the MAPE-K feedback control loop~\cite{kephart2003vision}. 
Based on the interactions between these components, Esfahani et al.~\cite{esfahani2013uncertainty} identify several sources of uncertainty, including:
\textit{simplified assumptions}, \textit{model drift}, \textit{noise}, \textit{parameters in future operation}, \textit{human in the loop}, \textit{objectives}, \textit{decentralization}, \textit{context}, and \textit{cyber-physical systems}.
%The User interacts with the Base-Level, providing expectations and setting objectives that guide the Meta-Level. 
%The Base-Level engages with entities in the Environment, while the Meta-Level, tasked with overseeing the Base-Level, consequently interacts with the Environment.  
Some of these Sources of Uncertainty are reused by Perez-Palacin et al.~\cite{perez2014uncertainties} and Mahdavi-Hezavehi et al.~\cite{mahdavi2017classification}. 
Instead of adding new uncertainty sources, Perez-Palacin et al.~\cite{perez2014uncertainties} classify existing sources from the literature according to their proposed taxonomy.
%The selection of sources focuses on the effect each source has on the model managed by a self-adaptive system (SAS). 
This classification aims at revealing similarities between the sources, making it possible to apply the same mitigation methods to similar types of uncertainty.
Mahdavi-Hezavehi et al.~\cite{mahdavi2017classification} offer an alternative understanding of uncertainty sources, defining them as circumstances that cause the system to diverge from its expected behavior.   
%Each category includes a brief description and examples, which incorporate some sources originally identified by Esfahani et al.~\cite{esfahani2013uncertainty}.

Bastin et al. ~\cite{bastin2013managing}, present two main origins of uncertainties: \textit{Model Input} and \textit{Model Structure}. 
Each source is further broken down into more granular sources. 
For \textit{Model Input}, these are \textit{Measurement Uncertainty}, \textit{Representativity Uncertainty}, \textit{Sensor Model Uncertainty}, and \textit{Transmission Uncertainty}. 
Correspondingly, the specific sources for \textit{Model Structure} uncertainty include \textit{Mechanism Uncertainty}, \textit{Representation Uncertainty}, \textit{Parameter Uncertainty}, and \textit{Numerical Uncertainty}. 

Zhang et al.~\cite{zhang2016understanding} introduce an alternative approach to defining an Uncertainty Source in the Belief Model, using the concept of \textit{Indeterminacy}. 
Indeterminacy describes a situation where current knowledge is insufficient to determine the actual state of a phenomenon.
Pared with Uncertainty, Indeterminacy describes the lack of confidence in a Belief Statement.
The explicit factors that contribute to this indeterminacy are referred to as \textit{Indeterminacy Sources}. 
Consequently, Zhang et al.~\cite{zhang2016understanding} define an Uncertainty Source as a subset of the sources of a belief statement, which lead to indeterminacy, e.g., the \textit{Indeterminacy Sources}.
Chatterjee et al.~\cite{chatterjee2020toward} adopt the same approach as Zhang et al.~\cite{zhang2016understanding}. 
The definition of Uncertainty Source is adopted within the Uncertainty Ontology presented by Bandyszak et al.~\cite{bandyszak2020orthogonal}, though they use the term \textit{Uncertainty Rationale} to refer to it. 

Bandyszak et al.~\cite{bandyszak2022uncertainty} present the ECDC (Execution platform, Communication infrastructure, Data processing, Coordination) reference model for characterizing uncertainty in real-time computing.
This model distinguishes various kinds of uncertainty based on four core concepts: \textit{Execution platform}, which includes the hardware and operating system for running real-time embedded software; \textit{Communication infrastructure}, referring to resources for data exchange and coordination between devices; \textit{Data Processing}, encompassing uncertainties in processing data from sensors or other technical devices; and \textit{Coordination}, addressing uncertainties from collaboration between autonomous systems.\\
Acosta et al.~\cite{acosta2022uncertainty} take a more abstract approach by differentiating between sources related to the system, such as the design, and those tied to the environment, including everything outside the boundary.\\  
Asmat et al.~\cite{asmat2023uncertainty} conduct a literature review specific to the domain of CPS, including approaches like the Belief Model by Zhang et al.~\cite{zhang2016understanding} and the Uncertainty Ontology from Bandyszack~\cite{bandyszak2020orthogonal}. 
The review results in a taxonomy of causes of uncertainty, which categorizes sources created from \textit{Human Behavior}, \textit{Natural Processes}, and \textit{Technological Processes}.

==> chapters/RelatedLiterature/types_old.tex <==
\subsection{Uncertainty Types}
\label{sec:uncertaintyTypes}
Zhang et al.~\cite{zhang2016understanding} introduce the concept of \textit{Uncertainty Types} within their Uncertainty Model. %, which expands upon uncertainty from multiple perspectives and establishes relevant abstractions.  
They define uncertainty as a state in which a "Belief Agent" lacks confidence in a "Belief Statement" and classify it into five types: \textit{Occurrence}, \textit{Environment}, \textit{Content}, \textit{Geographical Location}, and \textit{Time Uncertainty}
Chatterjee et al.\cite{chatterjee2020toward} and the PSUM-Metamodel~\cite{PSUM2023} adopt the different Uncertainty Types. \\% proposed in the Uncertainty Model by Zhang et al.~\cite{zhang2016understanding}.\\
Troya et al.\cite{troya2021uncertainty} also discuss uncertainty types in their survey. 
They review various approaches to represent uncertainty in software models, including the Uncertainty Model from Zhang et al.~\cite{zhang2016understanding}.
Their analysis results in a taxonomy of the following six uncertainty types: \textit{Spatiotemporal-}, \textit{Measurement-}, \textit{Occurrence-}, \textit{Design-}, \textit{Behavior-}, and \textit{Belief-Uncertainty}.

One uncertainty type that both Zhang et al.~\cite{zhang2016understanding} and Troya et al.~\cite{troya2021uncertainty} have in common is \textit{Occurrence Uncertainty}.
For Zhang et al.~\cite{zhang2016understanding}, it refers to a situation where a Belief Agent lacks confidence in the occurrence of events described in a Belief Statement. 
Troya et al.~\cite{troya2021uncertainty} focus on the occurrence of an entity rather than events.
Zhang et al.~\cite{zhang2016understanding} define the situation when the Belief Agent lacks confidence about the geographical location as \textit{Geographical Location Uncertainty}, and the lack of confidence about the time exiting in a Belief Statement as \textit{Time Uncertainty}. 
These two Uncertainty are combined by Troya et al.\cite{troya2021uncertainty} into \textit{Spatiotemporal Uncertainty}.

Various types of uncertainty are unrelated to each other. 
For instance, Zhang et al.~\cite{zhang2016understanding} interpretation includes \textit{Environment Uncertainty}, which represents a situation whereby a Belief Agent lacks confidence in the surroundings of a physical system existing in a Belief Statement, and \textit{Content Uncertainty}, which refers to the situation when the Belief Agent lacks confidence in the content existing in a Belief Statement.

Similarly Troya et al.~\cite{troya2021uncertainty} present various unrelated types of uncertainty: 
\textit{Measurement Uncertainty} refers to the set of possible states or outcomes of a measurement, with probabilities assigned to each state or outcome.
%Normally, these values are represented as primitive datatypes.  
\textit{Design Uncertainty} refers to a set of possible decisions or system design options. 
This uncertainty includes the usual developer's uncertainty about user requirements, their precision, and the system's operating conditions.
\textit{Behavior Uncertainty} refers to the lack of knowledge about the system or environment's behavior, including the actions, motivations, actual parameters, and timing.
\textit{Belief Uncertainty} exists when a belief agent is uncertain about any of the statements made in the model about the system or its environment. 

==> chapters/chapter3_jma.tex <==
\input{tables/literatureOverview}
\section{Overview of the related Literature}~\label{sec:literatureReview}
The objective of the literature review is to identify and analyze the most relevant uncertainty representations for the domain of Cyber-Physical Systems.
%not to achieve an exhaustive survey of all existing models. 
%Instead, we focus on identifying and analyzing the most prominent and relevant uncertainty representations that can be applied to the context of Cyber-Physical Systems. 
Rather than offering an exhaustive survey, we focus on key contributions that provide a representative overview of the current state of the art.
%By concentrating on these key representations, we aim to provide a representative and insightful overview of the current state of the art without diving into a comprehensive review of all the existing literature.
A complete list of all the literature included in the review can be found in Table \ref{tab:literatureOverview}.\\
This selection was made by including papers from various relevant domains, focusing on the domains of Software Engineering, Cyber-Physical Systems, and Coupled Models.
These domains were selected based on their contributions to understanding and managing uncertainty in Cyber-Physical Systems.
The subsequent sections of this chapter categorize the literature according to the dimensions or categories used to classify and represent uncertainty in the literature.
\subsection{Location}~\label{sec:location}
A total of nine papers address a category concerning the location of uncertainty in the representation of uncertainty. 
In the following paragraphs, we will explore the various definitions of uncertainty location.
\subsubsection{\citetitle{pelz2021mastering}}
Pelz et al.~\cite{pelz2021mastering} introduce the category \textit{System Design} to identify where uncertainties occur. 
This category consists of three distinct types of uncertainty: \textit{Data Uncertainty}, \textit{Model Uncertainty}, and \textit{Structural Uncertainty}.
\textit{Data Uncertainty} arises when there is a lack of completeness, clarity, or sufficiency in the required data's amount, type, or distribution.
\textit{Model Uncertainty} describes the situation when the functional relationships among input and output variables, model parameters, and other internal variables are either unknown, incomplete, inadequate, or unreasonable.
\textit{Structural Uncertainty} refers to the insufficient understanding of various possible function structures and the elements that generate them.
\subsubsection{\citetitle{perez2014uncertainties}}
Perez-Palacin et al.~\cite{perez2014uncertainties} define the point within a model where uncertainty manifests as the location of uncertainty.
%The location of uncertainty is described by Perez-Palacin et al.~\cite{perez2014uncertainties} as the point within the model where uncertainty manifests.
The presented options for the location of uncertainty in a model are \textit{Context}, \textit{Model structural}, and \textit{Input}. 
\textit{Context uncertainty} concerns the completeness of the model concerning the real world, e.g., inclusion and exclusion criteria.  
Concerns regarding the form of the model itself are grouped under the term \textit{Model structural uncertainty}. 
The more accurately the model represents the modeled subset of the real world, the less Model structural uncertainty exists. 
\textit{Input uncertainty}, also called parameter uncertainty, is all the uncertainty concerning the actual values of variables given as input to the model or variable calibrating methods.
\subsubsection{\citetitle{acosta2022uncertainty}}
The two understandings of Pelz et al.~\cite{pelz2021mastering} and Perez-Palacin et al.~\cite{perez2014uncertainties} about the location of uncertainty are combined by Acosta et al. ~\cite{acosta2022uncertainty} into a new notion called \textit{locus}.
'Locus' specifies which model elements are affected (locus) and the 'location in the real world'.
The different categories of the locus of uncertainty are \textit{Parameters}, \textit{Models}, \textit{Analysis}, and \textit{Decision Making}. 
\textit{Parameter uncertainty} includes uncertainties related to all types of parameters that characterize a model.
Uncertainty related to the model definition, formalism selection, boundaries, and structure are combined in the category \textit{Models}.
The category \textit{Analysis} comprises uncertainty from evaluating design decisions through model-based methods. 
This uncertainty arises from model abstractions and may be exacerbated by inaccuracies in analysis algorithms, such as approximations.
Uncertainties in the category \textit{Decision-Making} relate to the decision-making process when different options are available or when the decision is based on incomplete information and only estimates of the values of interest are available.
\subsubsection{\citetitle{zhang2016understanding}}
Zhang et al.\cite{zhang2016understanding} use the concept of belief statement to specify the location of uncertainty. 
A belief statement is a concrete and explicit specification of some belief held by a belief agent about possible phenomena or notions belonging to a given subject area.
Building on this concept, the location of uncertainty is defined by Zhang et al.\cite{zhang2016understanding} as the particular place or position where uncertainty occurs in such a Belief Statement. 
\subsubsection{\citetitle{walker2003defining}}
In their work, Walker et al.~\cite{walker2003defining} define the location of uncertainty as the point of manifestation within a complex model.
%identification of where the uncertainty manifests itself within the model complex. 
The location description in the model will vary according to the considered system model. 
Ideally, location description helps identify where the uncertainty affecting the outcome is created in the model.
Walker et al.~\cite{walker2003defining} list some of the most common locations that can be applied to most models: \textit{Context, Model Uncertainty, Inputs, Parameter Uncertainty, and Model Outcome Uncertainty}.
\textit{Context} identifies the system's boundaries, defining what is inside and outside and how fully it represents the real world.
The conceptual model, which defines the variables and relationships within the system, and the computer model are both associated with \textit{Model uncertainty}.
%\textit{Model uncertainty} arises from both the conceptual model, which defines the variables and relationships within the system, and the computer model. 
\subsubsection{\citetitle{chipman2015coverage}}
Chipman et al.~\cite{chipman2015coverage} base their definition of uncertainty location on the definition of Walker et al.~\cite{walker2003defining}, yet they choose a slightly different categorization. 
Instead of five types of location uncertainty,  Chipman et al.~\cite{chipman2015coverage} uses three different types: \textit{Input}, \textit{Parameters}, and \textit{Models}.
%Categories for the Location of an Uncertainty presented by \citetitle{chipman2015coverage} are \textit{Input-, Parameters-, and Modeling Uncertainties}. 
\textit{Input Uncertainties} are usually caused by the lack of knowledge of initial operating conditions or unforeseen scenarios. 
Values where the accurate values are unknown are grouped by the category \textit{Parameter Uncertainties}. For some of these values, statistical knowledge or a range from which the values are chosen is available.
\textit{Modeling uncertainties} contains uncertainties regarding the representation of an existing system.
\subsubsection{\citetitle{mahdavi2017classification}}
Mahdavi-Hezavehi et al.~\cite{mahdavi2017classification} define the location of uncertainty as the specific location within the whole system where uncertainty manifests.
Possible locations for uncertainty include \textit{Environment, Model, Adaption functions, Goals, Managed systems, and Resources}. 
\textit{Environment} includes the execution context and humans interacting with or affecting the system.
The Option \textit{Model} refers to various conceptual models representing the system. 
Functionalities performed as part of MAPE-K~\cite{kephart2003vision} are referred to as the option \textit{Adaptation functions}. 
The specification, modeling, and alternation of system goals are grouped under \textit{Goals}. 
All application-specific systems being monitored and adapted are organized as Option \textit{Managed Systems}.
\textit{Resources} refers to a variety of essential factors and components required by the self-adaptive system to operate normally.
\textit{Model uncertainty} can be divided into model structure uncertainty concerning the model's form and technical uncertainty related to its computer implementation.
\textit{Model inputs} are related to the description of the reference system, often the current system, and the external forces driving its changes.
The data and the methods to calibrate the model parameters are associated with \textit{Parameter Uncertainty}. 
%\textit{Parameter Uncertainty} refers to the data and the methods used to calibrate the model parameters
Uncertainty related to the model outcomes that are significant to the decision-maker is referred to as \textit{Model outcome uncertainty}.
%\textit{Model outcome uncertainty} refers to uncertainty related to the model outcomes of interest to the decision-maker.
\subsubsection{\citetitle{bandyszak2020orthogonal}}
Bandyszak et al.~\cite{bandyszak2020orthogonal} use the term "Observation Point" to document the artifacts that contain uncertainty and serve as locations where the system can detect this uncertainty.
Each observation point may be associated with multiple data sources.
\subsection{Source}\label{sec:source}
The following category used to represent uncertainty is called \textit{Uncertainty Source}. Also, this category is used by nine of the considered papers. 
\subsubsection{\citetitle{esfahani2013uncertainty}}
Esfahani et al.~\cite{esfahani2013uncertainty} use concepts from FORMS~\cite{weyns2010forms}, a reference architecture for self-adaptive software systems, to define the sources of uncertainty in the domain of self-adaptive systems. 
FORMS breaks down a self-adaptive system into the Base-Level, the main functionalities of a system, and the Meta-Level, which manages the Base-Level its behavior by using the MAPE-K feedback control loop~\cite{kephart2003vision}. 
In addition to the system's Meta- and Base-Level, Esfahani et al.'s model introduces two other key players: the User and the Environment. 
The User interacts with the Base-Level, providing expectations and setting objectives that guide the Meta-Level. 
The Base-Level engages with entities in the Environment, while the Meta-Level, tasked with overseeing the Base-Level, consequently interacts with the Environment. 
These interactions across different components introduce distinct uncertainty sources in self-adaptive systems.
Some examples of Uncertainty Sources mentioned by Esfahani et al. are:\textit{simplified assumptions}, \textit{model drift}, \textit{noise}, \textit{parameters in future operation}, \textit{human in the loop}, \textit{objectives}, \textit{decentralization}, \textit{context}, \textit{Cyber-physical systems}. 
%Uncertainty due to \textit{Simplifying Assumptions} comes to life from inaccuracies in the analytical models of the Meta-Level that manage the base-level subsystem. 
%Errors in predictions about adaptation impacts on quality attributes increase when these modeling abstractions fail to accurately capture the system.
%The uncertainty source \textit{Model Drift} arises when the meta-level subsystem’s decision-making models become inaccurate representations of the base-level subsystem due to loose coupling. 
%Additionally, adaptations may not be executed exactly as intended, causing these models to drift from the actual state of the base-level subsystem.
%Uncertainty due to \textit{Noise} arises from variations in monitored parameters, where the observed values typically form a range rather than a single value. 
\subsubsection{\citetitle{mahdavi2017classification}}
For Mahdavi-Hezavehi et al.~\cite{mahdavi2017classification}, the source of uncertainty describes circumstances influencing the adaptation decisions, which ultimately lead to deviations in the system performance from the expected behavior, e.g., circumstances that lead to uncertainties. 
Similar sources are categorized into classes, with Mahdavi-Hezavehi et al.~\cite{mahdavi2017classification} identifying six key groups: \textit{Model uncertainty}, \textit{Adaptation functions uncertainty}, \textit{Goals uncertainty}, \textit{Environment uncertainty}, \textit{Resources uncertainty}, and \textit{Managed system uncertainty}.
%possible to add examples for each group 
\subsubsection{\citetitle{perez2014uncertainties}}
Perez-Palacin et al.~\cite{perez2014uncertainties} classify uncertainty sources found in the literature regarding their impact on a model managed by the self-adaptive system~(SAS). 
The base of this classification is a taxonomy of uncertainties in SAS by Perez-Palacin et al.~\cite{perez2014uncertainties} with the following categories: nature, level, and location. 
The taxonomy aims to reveal similarities between different sources of uncertainty, particularly concerning applicable mitigation techniques.
Considered sources are \textit{Simplifying assumptions, Model drift, Noise in sensing, Future parameters value, Human in the loop, Objectives, Decentralization, Execution context/Mobility, Cyber-physical systems, Automatic learning, Rapid evolution, Granularity of models, and Different sources of information}. 
\subsubsection{\citetitle{bastin2013managing}}
According to  Bastin et al.~\cite{bastin2013managing} there are two primary origins of uncertainties: \textit{Model Input} and \textit{Model Structure}. 
Each primary source has a fine, granular selection of more specific sources. 
For \textit{Model Input}, these more specific sources are \textit{measurement uncertainty}, \textit{representativity uncertainty}, \textit{sensor model uncertainty}, and \textit{transmission uncertainty}. 
Respectively, for model structure uncertainty, the specific sources are \textit{mechanism uncertainty}, \textit{representation uncertainty}, \textit{parameter uncertainty}, and \textit{numerical uncertainty}.
\subsubsection{\citetitle{zhang2016understanding}}
Zhang et al.~\cite{zhang2016understanding} introduce a different concept to define the Uncertainty Source, referred to as \textit{Indeterminacy}. 
%explicitly describe the situation leading to uncertainty and stands for the explicit factors that lead to the situation where the information required to obtain the validity of a Belief Statement is unavailable. 
This term describes a situation in which the current knowledge is insufficient to determine the actual state of a phenomenon.
The factors that explicitly contribute to this Indeterminacy are termed Indeterminacy and are called Indeterminacy Sources. 
Consequently, Zhang et al.~\cite{zhang2016understanding} define an Uncertainty Source as a subset of the Sources of a Belief Statement, which leads to the source being Indeterminacy.















\subsection{Uncertainty Types}~\label{sec:uncertaintyTypes}
\subsection{Time}~\label{sec:time}
\subsection{Level}~\label{sec:level}
\subsection{Uncertainty Effect}\label{sec:effect}
\subsection{Pattern}~\label{sec:pattern}
\subsection{Type of Model}\label{sec:modelType}
\subsection{Nature}\label{sec:nature}






\textcolor{red}{First draft Johannes and Maribel}


\subsection{Identified Gaps and Limitations}~\label{sec:gapsLimitations}
\textcolor{red}{First draft Johannes +Maribel, extended by Raffaela and Diego}
- jungle of terminlogy 
- different terms for the same thing 



==> tables/literatureOverviewAlternative.tex <==
\begin{table}[!ht]
\centering
\caption{Overview of used Literature and its Uncertainty Categories}
\label{tab:literatureOverview}
\begin{tabular}{|p{2.6cm}|>{\centering\arraybackslash}m{0.7cm}|>{\centering\arraybackslash}m{1.1cm}|>{\centering\arraybackslash}m{0.8cm}|>{\centering\arraybackslash}m{0.7cm}|>{\centering\arraybackslash}m{0.9cm}|>{\centering\arraybackslash}m{0.7cm}|>{\centering\arraybackslash}m{0.6cm}|>{\centering\arraybackslash}m{0.6cm}|>{\centering\arraybackslash}m{0.7cm}|>{\centering\arraybackslash}m{0.5cm}|>{\centering\arraybackslash}m{0.5cm}|}
\hline
\footnotesize{\textbf{Paper}} & \footnotesize{\textbf{Source}} & \footnotesize{\textbf{Location}} & \footnotesize{\textbf{Nature}} & \footnotesize{\textbf{Model}} & \footnotesize{\textbf{Pattern}} & \footnotesize{\textbf{Effect}} & \footnotesize{\textbf{Level}} & \footnotesize{\textbf{Time}} & \footnotesize{\textbf{Types}}& \footnotesize{\textbf{Risk}}& \footnotesize{\textbf{Mitigation}}\\ \hline
\scriptsize{\citetitle{mahdavi2017classification}} & \multirow{6}{*}{\centering$\checkmark$} & \multirow{6}{*}{\centering$\checkmark$}  & \multirow{6}{*}{\centering$\checkmark$} &  &  &  &  \multirow{6}{*}{\centering$\checkmark$} & \multirow{6}{*}{\centering$\checkmark$} & &  &\\ \hline
\scriptsize{\citetitle{bandyszak2020orthogonal}} & \multirow{4}{*}{\centering$\checkmark$} & \multirow{4}{*}{\centering$\checkmark$} &  &  & \multirow{4}{*}{\centering$\checkmark$} &  \multirow{4}{*}{\centering$\checkmark$} &  &  & &  &\\ \hline
\scriptsize{\citetitle{pelz2021mastering}} &  & \multirow{2}{*}{\centering$\checkmark$} &  &  &  & \multirow{2}{*}{\centering$\checkmark$} &  &  & &  &\\ \hline
\scriptsize{\citetitle{walker2003defining}} &  & \multirow{5}{*}{\centering$\checkmark$} & \multirow{5}{*}{\centering$\checkmark$} &  &  &  & \multirow{5}{*}{\centering$\checkmark$} &  & & & \\ \hline
\scriptsize{\citetitle{perez2014uncertainties}} & \multirow{5}{*}{\centering$\checkmark$} & \multirow{5}{*}{\centering$\checkmark$} & \multirow{5}{*}{\centering$\checkmark$} &  &  &  & \multirow{5}{*}{\centering$\checkmark$} &  & & & \\ \hline
\scriptsize{\citetitle{bandyszak2022uncertainty}} & \multirow{2}{*}{\centering$\checkmark$} &  &  &  &  &  &  &  & & & \\ \hline
\scriptsize{\citetitle{esfahani2013uncertainty}} & \multirow{3}{*}{\centering$\checkmark$} &  &  &  &  &  &  &  & & & \\ \hline
\scriptsize{\citetitle{ramirez2012taxonomy}} &  &  &  &  &  &  &  & \multirow{3}{*}{\centering$\checkmark$} & & & \\ \hline
\scriptsize{\citetitle{bastin2013managing}} & \multirow{4}{*}{\centering$\checkmark$} &  &  &  &  &  &  &  & &  &\\ \hline
\scriptsize{\citetitle{acosta2022uncertainty}} & \multirow{3}{*}{\centering$\checkmark$} & \multirow{3}{*}{\centering$\checkmark$} &  & \multirow{3}{*}{\centering$\checkmark$} &  & \multirow{3}{*}{\centering$\checkmark$} &  & \multirow{3}{*}{\centering$\checkmark$} &  & & \\ \hline
\scriptsize{\citetitle{troya2021uncertainty}} &  &  &  &  &  &  &  &  & \multirow{3}{*}{\centering$\checkmark$} &  &\\ \hline
\scriptsize{\citetitle{chipman2015coverage}} &  & \multirow{2}{*}{\centering$\checkmark$} &  &  & \multirow{2}{*}{\centering$\checkmark$} & \multirow{2}{*}{\centering$\checkmark$} &  &  & &  &\\ \hline
\scriptsize{\citetitle{bertoa2020incorporating}} &  &  &  &  &  &  &  &  & & & \\ \hline
\scriptsize{\citetitle{zhang2016understanding}} & \multirow{4}{*}{\centering$\checkmark$} & \multirow{4}{*}{\centering$\checkmark$} &  &  & \multirow{4}{*}{\centering$\checkmark$} & \multirow{4}{*}{\centering$\checkmark$} &  & \multirow{4}{*}{\centering$\checkmark$} & \multirow{4}{*}{\centering$\checkmark$}& \multirow{4}{*}{\centering$\checkmark$} &\\ \hline
\scriptsize{\citetitle{chatterjee2020toward}} &  &  &  &  & \multirow{3}{*}{\centering$\checkmark$} &  &  &  & & & \\ \hline
\end{tabular}
\end{table}





==> tables/terminologyStatistics.tex <==
\begin{table}[[t!]]
\begin{center}
\caption{Statistics of Terminology in the Literature}
\label{tab:terminologyStatistics}
\begin{tabular}{|l|l|l|l|l|}
\hline
Category & $\#$ Catgeories & $\#$ Categories Names & $\#$ Category options & $\#$ Category options meanings \\ \hline
         &                      &                            &                            &                                     \\ \hline
         &                      &                            &                            &                                     \\ \hline
         &                      &                            &                            &                                     \\ \hline
         &                      &                            &                            &                                     \\ \hline
         &                      &                            &                            &                                     \\ \hline
         &                      &                            &                            &                                     \\ \hline
         &                      &                            &                            &                                     \\ \hline
         &                      &                            &                            &                                     \\ \hline
         &                      &                            &                            &                                     \\ \hline
         &                      &                            &                            &                                     \\ \hline
         &                      &                            &                            &                                     \\ \hline
         &                      &                            &                            &                                     \\ \hline
         &                      &                            &                            &                                     \\ \hline
         &                      &                            &                            &                                     \\ \hline
\end{tabular}
\end{center}
\end{table}
